Optimal and Efficient Dynamic Regret Algorithms for Non-Stationary Dueling Bandits

We study the problem of \emph{dynamic regret minimization} in $K$-armed Dueling Bandits under non-stationary or time varying preferences. This is an online learning setup where the agent chooses a pair of items at each round and observes only a relative binary `win-loss' feedback for this pair, sampled from an underlying preference matrix at that round. We first study the problem of static-regret minimization for adversarial preference sequences and design an efficient algorithm with $O(\sqrt{KT})$ high probability regret. We next use similar algorithmic ideas to propose an efficient and provably optimal algorithm for dynamic-regret minimization under two notions of non-stationarities. In particular, we establish $\tO(\sqrt{SKT})$ and $\tO({V_T^{1/3}K^{1/3}T^{2/3}})$ dynamic-regret guarantees, $S$ being the total number of `effective-switches' in the underlying preference relations and $V_T$ being a measure of `continuous-variation' non-stationarity. The complexity of these problems have not been studied prior to this work despite the practicability of non-stationary environments in real world systems. We justify the optimality of our algorithms by proving matching lower bound guarantees under both the above-mentioned notions of non-stationarities. Finally, we corroborate our results with extensive simulations and compare the efficacy of our algorithms over state-of-the-art baselines.

==> adv_db.tex <==
\section{\algp{} AND STATIC REGRET}
\label{section:3p}

This section describes our base algorithm \algp{} and a high-probability \emph{Static Regret} upper bound on its regret with respect to any fixed benchmark $i^* \in [K]$ (see $\sreg_T$, Sec. \ref{sec:prob}).

% ================================ %

\begin{algorithm}[h]
  \caption{\algp{}}
  \label{alg:3p}
  \begin{algorithmic}[1]
      \State \textbf{Input:} $\eta > 0$, $\gamma, \beta \in (0, 1)$
      \State Set $W_{+1, 1}(k) = W_{-1, 1}(k) = 1$ for all $k \in [K]$
      \For {$t = 1, \dots, T$}
        \For {$k \in [K]$ and $i \in \{+1, -1\}$}
          \State $p_{i, t}(k) = (1 - \gamma) \frac{W_{i, t}(k)}{\sum_{j=1}^K W_{i, t}(j)} + \frac{\gamma}{K}$
        \EndFor
        \State \multiline{For $i \in \{+1, -1\}$, sample $k_{i, t}$ from the distribution $(p_{i, t}(1), \dots, p_{i, t}(K))$ }
        \State Observe preference feedback $o_t(k_{+1, t}, k_{-1, t})$
        \State \multiline{Compute $\hat{g}_{i, t}(k)$ for $i \in \{+1, -1\}$ and $k \in [K]$ using \eqref{eq:hat_g}}
        \For {$k \in [K]$ and $i \in \{+1, -1\}$}
          \State $W_{i, t + 1}(k) = W_{i, t}(k) e^{\eta \hat{g}_{i, t}(k)}$
        \EndFor
      \EndFor
  \end{algorithmic}
\end{algorithm}

\subsection{\algp{} Algorithm}
\label{section:3p_algorithm}

Algorithm \ref{alg:3p} presents the pseudocode for \algp{}. It pits two players against each other, each parallely running its own copy of the standard EXP3 algorithm \citep{auer+02N}, the idea is famously introduced as sparring technique by \cite{Ailon+14} (see more discussions on similar works in Sec. \ref{sec:rel}). We refer to these players as the \textit{row player} and the \textit{column player}, and denote them by $+1$ and $-1$, respectively. 

As in EXP3, these players use weights, $\{W_{+1, t}(k)\}_{k=1}^K$ and $\{W_{-1, t}(k)\}_{k=1}^K$, to compute distributions over $K$ arms, $\bfp_{+1, t} = (p_{+1, t}(1), \dots, p_{+1, t}(K))$ and $\bfp_{-1, t} = (p_{-1, t}(1), \dots, p_{-1, t}(K))$ (Line 5), from which their actions are sampled (Line 7). We use $k_{+1, t}$ and $k_{-1, t}$ to denote the arms chosen by the row and column player at time $t$. The players then update their weights using the observed preference feedback $o_t(k_{+1, t}, k_{-1, t})$ that identifies the winner of a duel between the chosen arms.

The row player considers $r_{+1, t} = o_t(k_{+1, t}, k_{-1, t})$ as its reward at time $t$ whereas the column player uses $r_{-1, t} = 1 - o_t(k_{+1, t}, k_{-1, t})$. The weight update for each player is similar to EXP3 (Line 11) and uses the following expression as an importance-weighted estimate of the rewards. For $i \in \{+1, -1\}$,
\begin{equation}
  \label{eq:hat_g}
  \hat{g}_{i, t}(k) = \begin{cases}
    (r_{i, t} + \beta) / p_{i, t}(k) & \text{if } k = k_{i, t} \\
    \beta / p_{i, t}(k) & \text{otherwise.}
  \end{cases}
\end{equation}
The quantity $\beta \in (0, 1)$ in the expression above prevents $\hat{g}_{i, t}(k)$ from becoming too large when $p_{i, t}(k)$'s are small. This is crucial for obtaining a high-probability regret guarantee (see proof of Lemma \ref{lemma:3p_bound_row_player} in Appendix \ref{appendix:3p_bound_row_player_proof}).

As both players try to maximize their cumulative rewards, they start putting a higher weight on arms that are more likely to win against the choice made by the opponent. An equilibrium is reached when both players choose the optimal arm. The quantity $\gamma \in (0, 1)$ in Line 5 ensures a minimum exploration of all arms and encourages the players to reach the optimal equilibrium strategy. Next, we establish a high-probability static regret guarantee for \algp{}.

% ================================ %

\subsection{Analysis: Static Regret Guarantee}
\label{section:3p_analysis}

Given the actions $\{k_{+1, t}, k_{-1, t}\}_{t=1}^T$ taken by the players, the total regret with respect to fixed action $j \in [K]$ is defined as:
\begin{equation*}
    \sreg_T(j) = \sum_{t=1}^T \frac{P_t(j, k_{+1, t}) + P_t(j, k_{-1, t}) - 1}{2}.
\end{equation*}

 The \emph{central idea} in our analysis is to decompose the total regret into the regret incurred by the row ($\sreg_T^{+1}(j)$) and the column ($\sreg_T^{-1}(j)$) player, defined as
\begin{align*}
    \sreg_T^{+1}(j) &= \sum_{t=1}^T P_t(j, k_{-1, t}) - P_t(k_{+1, t}, k_{-1, t}) \\
    \sreg_T^{-1}(j) &= \sum_{t=1}^T P_t(j, k_{+1, t}) - P_t(k_{-1, t}, k_{+1, t}).
\end{align*}
It is easy to see that $\sreg_T(j) = \frac{1}{2} \left( \sreg_T^{+1}(j) + \sreg_T^{-1}(j) \right)$. The next two lemmas establish high-probability upper bounds on $\sreg_T^{+1} \coloneqq \max_{j \in [K]} \sreg_T^{+1}(j)$ and $\sreg_T^{-1} \coloneqq \max_{j \in [K]} \sreg_T^{-1}(j)$.

\begin{restatable}{lemma}{algprowplayer}
  \label{lemma:3p_bound_row_player}
  Let $\eta = \frac{1}{2}\sqrt{\frac{\ln K}{KT}}$, $\beta = \sqrt{\frac{\ln K}{KT}}$, and $\gamma = 2\eta K \geq (1 + \beta) \eta K$. With probability at least $1 - \delta$, 
  $$\sreg_T^{+1} \coloneqq \max_{j\in [K]} \sreg_T^{+1}(j) = O(\sqrt{KT} \ln (K/\delta)).$$
\end{restatable}

\begin{restatable}{lemma}{algpcolumnplayer}
  \label{lemma:3p_bound_column_player}
  Let $\eta$, $\beta$, and $\gamma$ be set as in Lemma \ref{lemma:3p_bound_row_player}. With probability at least $1 - \delta$, 
  $$\sreg_T^{-1} \coloneqq \max_{j\in [K]} \sreg_T^{-1}(j) = O(\sqrt{KT} \ln (K/\delta))$$
\end{restatable}

The following regret bound on $\max_{j \in [K]} \sreg_T(j)$ is now a straightforward consequence of the two lemmas above.

\begin{restatable}[Static-Regret of \algp]{theorem}{algpanalysis}
  \label{theorem:3p_bound}
Set $\eta$, $\beta$, $\gamma$ as in Lem. \ref{lemma:3p_bound_row_player}. Then with probability at least $1 - 2\delta$
  $$\max_{j \in [K]} \sreg_T(j)[\algp{}] = O\left(\sqrt{KT} \ln \left( \frac{K}{\delta} \right) \right)$$
\end{restatable}

Lemmas \ref{lemma:3p_bound_row_player} and \ref{lemma:3p_bound_column_player} have been proved in Appendix \ref{appendix:3p_analysis}. \emph{From the perspective of each agent, the actions of other agents, and hence their own rewards, are adaptively chosen by an adversary.} With this insight, one can borrow techniques from the analysis of the standard EXP3 algorithm to establish the high-probability regret bound in Thm. \ref{theorem:3s_bound}.

\begin{remark}
\label{rem:exp3p}
  The regret guarantee above has been written in terms of any fixed (pure) action $j \in [K]$ in hindsight. However, the adversary can also play any fixed distribution over actions $\bmpi^* \in \Delta_K$, and the same regret guarantee will be valid against $\bmpi^*$. Consequently, this implies that our algorithm achieves an $\tO(\sqrt{KT})$ regret w.r.t. the Nash-Equilibrium (alternative termed as the Von-Neumann winner \footnote{Given a preference matrix $\P$, a Von-Neumann winner of $\P \in [0,1]^{K \times K}$ is defined to be a probability distribution $\pi \in \Delta_{K}$, such that
$
\sum_{i=1}^{n} \pi(i)P(i,b) \ge 1/2, ~~\forall b \in [K]. 
$ (see Eqn. $1$, \citep{dudik+15})}) of the aggregated matrix $\frac{\big(\sum_{t =1}^T \P_t \big)}{T}$, or even against the best response $\bmpi^*:= \arg\max_{\pi \in \Delta_K}\sreg_T(\pi)[\algp]$.
\end{remark}

With the base algorithm in place, we now modify \algp{} to obtain \algs{} and derive high-probability dynamic regret guarantees for this algorithm.% in the next section.

% ================================ %


==> ub.tex <==
\begin{algorithm}[t]
  \caption{\algs{}}
  \label{alg:3s}
  \begin{algorithmic}[1]
      \State \textbf{Input:} $\eta > 0$, $\alpha, \gamma, \beta \in (0, 1)$
      \State Set $W_{+1, 1}(k) = W_{-1, 1}(k) = 1$ for all $k \in [K]$
      \For {$t = 1, \dots, T$}
        \For {$k \in [K]$ and $i \in \{+1, -1\}$}
          \State $p_{i, t}(k) = (1 - \gamma) \frac{W_{i, t}(k)}{\sum_{j=1}^K W_{i, t}(j)} + \frac{\gamma}{K}$
        \EndFor
        \State \multiline{For $i \in \{+1, -1\}$, sample $k_{i, t}$ from the distribution $(p_{i, t}(1), \dots, p_{i, t}(K))$ }
        \State Observe preference feedback $O_t(k_{+1, t}, k_{-1, t})$
        \State \multiline{Compute $\hat{g}_{i, t}(k)$ for $i \in \{+1, -1\}$ and $k \in [K]$ using \eqref{eq:hat_g}}
        \For {$k \in [K]$ and $i \in \{+1, -1\}$}
          \State \small{$W_{i, t + 1}(k) = W_{i, t}(k) e^{\eta \hat{g}_{i, t}(k)} + e \alpha \sum_{j=1}^K W_{i, t}(j)$}
        \EndFor
      \EndFor
\end{algorithmic}
\end{algorithm}

\section{\algs{} AND DYNAMIC REGRET}
\label{section:3s}

Competing against a fixed action in hindsight is an interesting but modest goal. In this section, we consider the dynamic regret objective  $\dreg_T(j^T)$ defined with respect to \emph{any sequence of actions} $j^T = (j_1, \dots, j_T)$ (see Section \ref{sec:prob}). It is clear that $\dreg_T(j^T)$ can be $O(T)$ in the worst case unless one imposes further assumptions. Sections \ref{section:switch_nonstationarity} and \ref{section:continuous_nonstationarity} respectively assume the `\sv' and `\cv' model of non-stationarity (see Section \ref{sec:prob}) to derive sub-linear dynamic regret guarantees.

To achieve these bounds, we propose \algs{}, a variant of \algp{}. This algorithm uses the same procedure as \algp{}, except at Line 11, where it instead uses the following weight update rule:
\begin{equation*}
  W_{i, t + 1}(k) = W_{i, t}(k) e^{\eta \hat{g}_{i, t}(k)} + e \alpha W_{i, t}.
\end{equation*}
Here, $\alpha \in (0, 1)$ is a user-specified hyper-parameter and $W_{i, t} \coloneqq \sum_{j=1}^K W_{i, t}(j)$. Algorithm \ref{alg:3s} presents this procedure. We next move to the analysis of \algs{} under the two non-stationarity models.

% ================================ %

\subsection{Dynamic Regret Analysis of \algs{} under \sv{} $S$}
\label{section:switch_nonstationarity}

As before, we write $\dreg_T(j^T)$ as $\dreg_T(j^T) = \frac{1}{2}(\dreg_T^{+1}(j^T) + \dreg_T^{-1}(j^T))$, where $\dreg_T^{+1}(j^T)$ and $\dreg_T^{-1}(j^T)$ is the dynamic regret incurred by the row and the column player with respect to the sequence $j^T$: %That is, 
\begin{align*}
  \dreg_T^{+1}(j^T) &= \sum_{t=1}^T P_t(j_t, k_{-1, t}) - P_t(k_{+1, t}, k_{-1, t}) \\
  \dreg_T^{-1}(j^T) &= \sum_{t=1}^T P_t(j_t, k_{+1, t}) - P_t(k_{-1, t}, k_{+1, t}).
\end{align*}
We assume that the sequence $j^T$ has at most $S$ switches, i.e., $1 + \abs{\lbrace 1 \leq \ell < T: j_\ell \neq j_{\ell + 1} \rbrace} \leq S$. The result below bounds $\dreg_T(j^T)$ under two conditions, first where $S$ is known to the algorithm apriori and second where it is unknown.

\begin{restatable}[\algs{} regret under \sv{}]{theorem}{algsanalysis}
  \label{theorem:3s_bound}
  Let $j^T = (j_1, \dots, j_T)$ be any arbitrary sequence of actions with $S$ switches. Then the following bounds hold for \algs{} with probability at least $1 - \delta$ when $\alpha = \frac{1}{T}$ and $\gamma = 2 \eta K$:
 
 (1) $\dreg_T(j^T)[\algs] = O \left( \sqrt{SKT} \ln \frac{KT}{\delta} \right)$, and

  (2) $\dreg_T(j^T)[\algs] = O \left( S \sqrt{KT} \ln \frac{KT}{\delta} \right)$, 
  by respectively setting $\beta = \eta = \sqrt{\frac{S}{KT}}$, and $\beta = \eta = \frac{1}{\sqrt{KT}}$.
\end{restatable}

In the first case above, $S$ is known apriori to the algorithm and is used for setting $\beta$ and $\eta$. If $S$ is unknown and the regret grows linearly with $S$.% instead of growing as $\sqrt{S}$. 

\begin{remark}
  \label{remark:optimal_jT}
  Theorem \ref{theorem:3s_bound} is valid for any sequence $j^T$ with $S$ switches. In particular, $j^T$ can be constructed as follows. \textbf{(i)} Divide the time horizon $T$ into $S$ sub-intervals $[T_1, \dots, T_2)$, $[T_2, \dots, T_3)$, \dots, $[T_S, \dots, T_{S + 1})$, where $T_1 = 1$ and $T_{S + 1} = T + 1$. \textbf{(ii)} Assume $P_{t}(i, j) = P^s(i, j)$ for all $t \in [T_s, T_{s + 1})$, $s \in [S]$, and $i, j \in [K]$. \textbf{(iii)} Set $j_{T_s} = j_{T_s + 1} = \dots = j_{T_{s + 1} - 1} = j^s$, where
  \begin{equation*}
    j^s = \argmax_{j \in [K]} \sum_{t = T_s}^{T_{s + 1} - 1} \frac{P^s(j, k_{+1, t}) + P^s(j, k_{-1, t}) - 1}{2}.
  \end{equation*}
  In other words, if the winner probabilities remain constant within sub-intervals $[T_s, T_{s + 1})$, then $j_{T_s}, \dots, j_{T_{s + 1} - 1}$ can be set to the best action within this sub-interval in hindsight for each $s \in [S]$. Theorem \ref{theorem:3s_bound} will be valid for such a sequence $j^T$. Therefore, if preferences $\bfP_1, \dots, \bfP_T$ have \sv{} $S$, then, with probability at least $1 - \delta$,
  \begin{align*}
    \dreg_T(j^1,\ldots,j^S)[\algs] = \begin{cases}
        O \left(  \sqrt{SKT} \ln \frac{KT}{\delta} \right),\\
        O \left( S\sqrt{KT} \ln \frac{KT}{\delta} \right), 
     \end{cases}
 \end{align*}
 for known and unknown $S$ respectively.
\end{remark}

\begin{remark}
\label{rem:exp3s_pi}
  As in \algp{}, the adversary can play a fixed distribution over actions in each of the sub-intervals $[T_s, T_{s + 1})$ instead of playing a single fixed action, as explained in Rem. \ref{rem:exp3p}. A similar regret guarantee as Theorem \ref{theorem:3s_bound} would still hold for \algs{}.
\end{remark}

The proof of Theorem \ref{theorem:3s_bound} uses the same regret decomposition strategy as was used in Theorem \ref{theorem:3p_bound}. Lemmas \ref{lemma:3s_row_player_bound} and \ref{lemma:3s_column_player_bound} in Appendix \ref{appendix:3s_analysis_switch} establish high-probability upper bounds on $\dreg_T^{+1}(j^T)$ and $\dreg_T^{-1}(j^T)$. Theorem \ref{theorem:3s_bound} then follows by combining the two lemmas. 

% \paragraph{Dynamic-Regret with \sv\, $(S)$. }
% A consequence of Thm. \ref{theorem:3s_bound} is, the dynamic regret of \algs{} on any non-stationary sequence $P_1,\ldots,P_T$ of \sv\, $S$ (Sec. \ref{sec:prob}), is bounded:

% \begin{restatable}[\algs\, with \sv]{theorem}{svalgsanalysis}
% \label{theorem:3s_bound}
% Consider any preference sequence $P_1,\ldots,P_T$ with \sv\, $S$. Then choosing the parameters as defined in Thm. \ref{theorem:3s_bound_timevar}, with probability at least $(1-\delta)$\\
%  $\dreg_T(\algs) = \begin{cases}
%  O \left(  \sqrt{SKT} \ln \frac{KT}{\delta} \right), \text{for known } S\\
%  O \left( S\sqrt{KT} \ln \frac{KT}{\delta} \right), \text{for unknown } S
%  \end{cases}$.
% \end{restatable}

% ================================ %


==> ub2.tex <==
\subsection{Dynamic Regret Analysis of \algs{} under \cv{} $V_T$}
\label{section:continuous_nonstationarity}

% Another extension of Thm. \ref{theorem:3s_bound_timevar}'s regret guarantee is to analyze the dynamic regret of \algs{} with respect to \cv\, non-stationarity (Sec. \ref{sec:prob}). 

One can decompose the dynamic regret along the same lines as in Section \ref{section:switch_nonstationarity} to establish a dynamic regret guarantee for \algs{} under the \cv{} model of non-stationarity (Sec. \ref{sec:prob}).

\begin{restatable}[\algs\, regret under \cv]{theorem}{cvalgsanalysis}
\label{theorem:3s_boundcv}
Consider any preference sequence $\bfP_1, \ldots, \bfP_T$ with \cv\, $V_T$. Then, setting $\alpha, \gamma$ same as defined in Thm. \ref{theorem:3s_bound} and $\beta = \eta = \frac{V_T^{1/3}}{4K^{2/3}T^{1/3}}$, for any time-variant benchmark $j^T=(j_1,\ldots,j_T)$, with probability at least $(1-\delta)$, the dynamic regret bound of \algs{} satisfies $\dreg_T(j^T)[\algs] = O\Big( \big(V_T^{1/3}K^{1/3}T^{2/3} + 4K^{2/3}T^{1/3}V_T^{-1/3} \big)\ln \frac{KT}{\delta}\Big)$.
\end{restatable}

The proof of Theorem \ref{theorem:3s_boundcv} mainly relies on the observation that for any sub-interval $\cI \subseteq [T]$ with limited \cv\, budget, the `performance-difference' between any fixed benchmark (arm) $j^* \in [K]$ vs a time-varying benchmark (say sequence of arms $\{j_\tau^*\}_{\tau \in \cI}$) is bounded. Hence, one can divide the full time horizon $[T]$ into small sub-intervals $\cI_1, \ldots, \cI_S$, each of length say $\Delta$ (a tuning parameter to be chosen appropriately), thus $S = \lceil T/\Delta\rceil$, and apply the results from Thm. \ref{theorem:3s_bound} to bound the learner's regret within each sub-interval (against a fixed benchmark). The bound in Thm. \ref{theorem:3s_boundcv} now follows by combining both these factors and by properly adjusting $\Delta$ along with the algorithm parameters $\alpha, \beta, \eta$, and $\gamma$. The complete proof is given in Appendix \ref{app:cont_nst}.

\begin{remark}
Theorems \ref{theorem:3s_bound} and \ref{theorem:3s_boundcv}, together with Theorems \ref{theorem:lower_bound_switch} and \ref{theorem:lower_bound_continuous} respectively, imeediately justify the optimality of \algs{} and tightness of our regret analysis in terms of Switching and Continuous Variation. 
\end{remark}

\begin{remark}
\label{rem:high_prob_to_expected_regret}
The regret guarantees in Theorems \ref{theorem:3p_bound}, \ref{theorem:3s_bound}, and \ref{theorem:3s_boundcv} hold with probability at least $1 - \delta$. The corresponding expected regret guarantees of the same order can be derived by setting $\delta = 1/T$. For example, against any sequence $j^T$ with \sv\, $S$, Thm. \ref{theorem:3s_bound} gives $\sreg_T[\algp{}] = O(\sqrt{KT}\ln KT)$ with probability $(1 - \delta)$, and $\sreg_T[\algp{}] \le T$ with probability $\delta$. Thus choosing $\delta = \frac{1}{T}$ one may conclude that $\rmE{\sreg_T[\algp{}]} = O(\sqrt{KT}\ln KT)$.
\end{remark}


